Detect-Localize-Repair: A Unified Framework for Learning to Debug with CodeT5

Automated software debugging is a crucial task for improving the productivity of software developers. Many neural-based techniques have been proven effective for debugging-related tasks such as bug localization and program repair (or bug fixing). However, these techniques often focus only on either one of them or approach them in a stage-wise manner, ignoring the mutual benefits between them. In this work, we propose a novel unified \emph{Detect-Localize-Repair} framework based on a pretrained programming language model CodeT5 to seamlessly address these tasks, named CodeT5-DLR. Specifically, we propose three objectives to adapt the generic CodeT5 for debugging: a bug detection objective to determine whether a given code snippet is buggy or not, a bug localization objective to identify the buggy lines, and a program repair objective to translate the buggy code to its fixed version. We evaluate it on each of these tasks and their combined setting on two newly collected line-level debugging datasets in Java and Python. Extensive results show that our model significantly outperforms existing baselines from both NLP and software engineering domains.

==> body.tex <==
%!TEX root=emnlp2022.tex
\section{Introduction}
\label{sec:intro}
\input{introduction}

% \section{Technical Detail}
% \label{sec:model}
\input{model_new}


\section{Evaluation}
\label{sec:eval}
\input{evaluation}




%	
%\end{acks}


==> evaluation.tex <==
%!TEX root=emnlp2022.tex
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\subsection{Datasets}

We collect 2 datasets, one is the single line bug-fixes pair and the other is the multi-line bug-fixes pair. The single line bug-fixes~\cite{karampatsis2020often} have been considered recently as one of the major issues that affect on the source code's quality and there are a number of datasets for such single line bug fixes~\cite{karampatsis2020often, richter2022tssb}. However, these datasets are not suitable for our purpose due to 2 reasons: (1) they contain only the code changes at the file level while our goal is to detect buggy lines at the function level and line level(2) they does not contain the before and after information of the code changes but they only contain the patches (difference between the before and after). With such reasons, we need to collect datasets by our own for evaluation.  We follow the steps from ~\cite{karampatsis2020often} to collect 2 datasets for 2 programming languages, one is for Java and the other is for Python.

\begin{enumerate}[leftmargin=*]
	\item Single line bug-fixes (SL-Java):  Single-line bug fixes have recently been identified as one of the major issues that have an impact on the quality of the source code~\cite{karampatsis2020often}. These bugs can be fixed easily with simple code changes such as changing the operator, renaming variables, and so on. However, these bugs occurred frequently, and current static-based techniques are incapable of detecting them accurately (accuracy 10\%). In the ManySStuBs4J~\cite{karampatsis2020often} dataset, such bug fixes have been studied and classified into 16 bug templates for Java. However, this dataset is insufficient for our needs for two reasons: (1) they only contain code changes at the file level, whereas our goal is to detect buggy lines at the function level; and (2) they do not contain before and after information about code changes, but only patches. For these reasons, we must collect our own datasets for evaluation. 
	\item Multi line bug-fixes in Python (ML-Python): In addition to the single line bug-fixes dataset, we also want to evaluate our technique to detect multi line bug-fixes. The multi line bug fixes are usually more challenging to detect and fix. It is not to de-emphasize the importance of single line bug-fixes bug to illustrate different real-world scenario when detect bugs. 
\end{enumerate}

To extract code changes from Github commits, we use Pydriller~\cite{Spadini2018}, a tool that mines software repositories from Git.  he code changes are made up of three parts of a source file: before changes, after changes, and the difference between the two (patch). However, because we want to localise bugs at the \textit{function and line level} rather than the file level, we need to perform additional preprocessing to extract the code changes at the \textit{function level}. We use Lizard~\footnote{https://github.com/terryyin/lizard, a code analysis tool to extract the functions from a file that works for multiple programming languages.} to extract the functions and compare the different between the functions from the before and after version of a source file (obtained from Pydriller). Figure~\ref{fig:sample} depicts a sample from our data collection process that was successfully extracted.

 For SL-Java, beside the code changes for bug fixes, we also follow ~\citet{karampatsis2020often} to use tree-sitter~\footnote{https://github.com/tree-sitter/tree-sitter} to identify 16 bug patterns for the single buggy lines. We do not aim to detect the exact but patterns because the patterns can be easily detected using matching rules on the Abstract Syntax Tree if we can localize if a line is buggy. The patterns, on the other hand, will be useful in analysing how well our techniques work on each pattern, allowing us to gain a better understanding of the difficulty in detecting each pattern.

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.99\textwidth]{figures/data_sample.png}
	\caption{An illustration of the appearance of an instance in our dataset. The code snippet on the left is the buggy code (before), with the line number of the buggy line indicated (line 5 in this case). The code snippet on the right represents the fixed code (after).}
	\label{fig:sample}
\end{figure*}

\input{tables/data_stats}
% \begin{table}[t]
% 	\centering
% 	\fontsize{8.5}{9.5}\selectfont 
	
	
% 	\caption{Statistics of our datasets}
% 	\begin{tabular}{|c|cc|cc|}
% 		\hline
% 		\multirow{2}{*}{} & \multicolumn{2}{c|}{SL-Java}                      & \multicolumn{2}{c|}{ML-Python}                     \\ \cline{2-5} 
% 		& \multicolumn{1}{c|}{Projects} &  Instances & \multicolumn{1}{c|}{ Projects} &   Instances \\ \hline
% 		Train             & \multicolumn{1}{c|}{2348}         & 56449         & \multicolumn{1}{c|}{3351}         & 132243        \\ \hline
% 		Test              & \multicolumn{1}{c|}{700}          & 16083         & \multicolumn{1}{c|}{867}         & 35457         \\ \hline
% 		Val               & \multicolumn{1}{c|}{335}          & 7865          & \multicolumn{1}{c|}{480}          & 22395         \\ \hline
% 	\end{tabular}
% \label{tab:dataset}
% \end{table}

Table~\ref{tab:dataset} shows the statistics of our datasets, which have been split into training, testing and validation parts. For function-level bug detection task, we use the whole code snippet . The buggy or non-buggy label is decided by simply treat the before version as the buggy (label 0) and the after version as non-buggy (label 1). 
For line-level bug localization task, we use the buggy line's number information to train the model to localize which line is buggy. For program repair, the before version is used as the source and the after version is used the the target.



\subsection{Model Implementations}

We employ the CodeT5-based (220M) as the foundation model for our neural architecture. We set the maximum source and target sequence lengths to 512. We train our model on a cluster of 16 NVIDIA A100 GPUs with 40 GB memory. 

% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



\subsubsection{Function-Level Bug Detection}
\paragraph{Metrics}
For this task, we use two metrics: the F1 score and the False Positive Rate (FPR). F1 is the standard metric for this type of task because it is a binary classification problem (buggy or not). The FPR, on the other hand, is critical for determining a bug localization system's usability in a real-world scenario. A good bug detection system should produce as few false positives as possible~\cite{allamanis2021self, vasic2019neural}.  The FPR is calculated as the ratio between the number of non-buggy functions wrongly categorized as buggy (false positives) and the total number of actual non-buggy functions. 

\paragraph{Baselines}
The function-level bug detection can be seen as a form of code classification task, in which we aim to assign a label to a given code snippet. As such, we choose Tree-based CNN~\cite{mou2016convolutional}, a well-known baseline for code classification. We also including some others SOTA  pretrained language models of code, which are CodeBERT~\cite{feng-etal-2020-codebert}, GraphCodeBERT~\cite{guo2020graphcodebert}, and PLBART~\cite{ahmad2021unified}. For these pretrained models, we used their public ptretrained models and fine-tune them for this task. We also include SpotBugs~\footnote{https://github.com/spotbugs/spotbugs}, a static analysis-based baseline that is widely used  as a baseline~\cite{karampatsis2020often, habib2018many} for bug detection task.

\paragraph{Results}

\input{tables/result_detect}

Table~\ref{tab:function_level} shows the results of function-level bug detection task. Our model fine-tuned with all 3 objectives together achieve the best performance in term of both F1 score and FPR. In addition we also fined-tune CodeT5 with only the function-level bug detection objective, the performance of CodeT5 is still the best among the baselines. The SpotBugs baseline achieves only 4.6 in F1 score, which is consistent with the performance reported in~\citet{habib2018many} for static analysis-based bug detector.
\subsubsection{Line-Level Bug Detection}
\paragraph{Metrics}
For this task, we use 3 metrics to evaluate the performance, which are Mean Reciprocal Rank (MRR), Mean Average Precision (MAP), and False Positive Rate (FPR).
Given that our goal is to retrieve the correct buggy lines from a list of all the lines in the source code snippet, we can formulate this problem as an information retrieval problem, with the goal of returning a ranked list of relevant lines to a query (given that a query is to retrieve all of the buggy lines among the lines). In this case, we use the well-known metrics of MRR and MAP to evaluate information retrieval systems. In our evaluation settings, each of these metrics will be appropriate for a different datasets. For the SL-Java, because there is only one buggy line in the ground truth, the MRR is appropriate for evaluating the performance of this task for the SL-Java dataset. On the other hand, each of sample in ML-Python contains numerous buggy lines in the ground truth, the MAP is better suited for ML-Python. However, in reality, we do not know how many lines of code is buggy, so we retrieve top-k lines with highest scores and measure if the ground-truth buggy lines(s) belong to these top-k lines. With this, MRR and MAP are computed with respect to $k$, resulting in MRR@k and MAP@k, where $k$ is number of lines retrieved for evaluation. We choose $k = 1$ and $k = 5$ for our evaluation. 

%\paragraph{Mean Reciprocal Rank} : The mean reciprocal rank is the average of the reciprocal ranks of results of a set of
%queries Q. The reciprocal rank of a query is the multiplicative inverse of the rank of the first correct answer. MRR can be calculated as follows:
%\begin{equation}
%	\small
%	MRR = \frac{1}{\mid Q\mid}\sum_{i=1}^{\mid Q\mid}\frac{1}{\mid rank_{i}\mid}
%\end{equation}
%
%\paragraph{Mean Average Precision} : Mean average precision (MAP) for a set of queries is the mean of the average precision scores for each query. MAP provides a single-figure measure of quality of information retrieval, when a query may have multiple relevant documents. The Average Precision (AveP) of a single query is the average of the precision values obtained for the query. MAP and AveP can be calculated as follows:
%\begin{equation}
%	\small
%	AveP = \frac{1}{\mid Q\mid}\sum_{i=1}^{\mid M\mid}\frac{1}{\mid rank_{i}\mid};
%	\\
%	MAP = \frac{\sum_{q=1}^{Q}AveP(q)}{Q}
%\end{equation}


In addition to MRR and MAP, we also use FPR to measure . Given a code snippet and retrieved buggy lines, the FPR in this case is calculated as the ratio between the number of non-buggy lines wrongly categorized as buggy (false positives) and the total number of actual non-buggy lines. We also compute FPR with respected to top-k lines retrieved, similar to MRR and MAP.
\paragraph{Baselines}

For this task, we also chose baselines that are similar to the Function-level bug localization task, which are CodeBERT~\cite{feng-etal-2020-codebert}, GraphCodeBERT~\cite{guo2020graphcodebert}, and PLBART~\cite{ahmad2021unified}. In addition, we include 2 additional baselines that have been used to detect vulnerability in software engineering, which are DeepLineDP~\cite{pornprasit2022deeplinedp} and LineVul~\cite{fu2022linevul}. They work by simply performing prediction at the function level, then using attention scores from the backbone neural architecture to retrieve the line scores to predict vulnerability at line level. DeepLineDP is based on the Hierrarchical Attention Network~\cite{yang2016hierarchical}, which divides the source code into three layers: function, line, and token, with each level processed by a BiGRU neural network. LineVul is based on a vanilla Transformer~\cite{vaswani2017attention}, and its scores are calculated by averaging the token scores from the multi head attention layer. DeepLineDP and LineVul has not been used for bug detection before, but we try our best to adapt their software artifacts~\footnote{https://github.com/awsm-research/DeepLineDP}~\footnote{https://github.com/awsm-research/LineVul} into our use case.

\paragraph{Results}

The results of line-level bug localization task is shown in Table~\ref{tab:line_level}.  When fine-tuning on all objectives, our model outperforms all baselines in terms of all metrics. The FPR is low when we only aim to detect one line of buggy code. When we increase k to 5, the FPR increases, which means. With k = 5, however, the MRR and MAP are better for either single-line bug detection (SL-Java) or multi-line bug detection (ML-Python). It means that as we broaden the scope of buggy line retrieval, the number of correctly detected bugs increases, but the model produces more false alarms. When performing bug localization at the line level, this is a trade off that must be made.

\input{tables/result_localize}
\subsubsection{Program Repair}
\paragraph{Metrics}
We use 2 metrics for program repair: Exact Match (EM) and BLEU. For EM, if the generated program exactly match the ground truth correct program, then EM=1, otherwise EM=0. BLEU score is a standard metric that is usually used to measure translation-based tasks.

\paragraph{Baselines}
We also use CodeBERT~\cite{feng-etal-2020-codebert}, GraphCodeBERT~\cite{guo2020graphcodebert}, and PLBART~\cite{ahmad2021unified} for the program repair task. We fine-tune these pretrained models with the Seq2Seq objective to generate the fixed code from buggy code.


\paragraph{Results}

Table~\ref{tab:program_repair} shows the results of program repair task. Our model when fine-tuning on all 3 objectives achieves the best performance among the baselines with significant margins, both in term of EM and BLEU. In overall, EM for ML-Python is lower than EM for SL-Java, it is because that it is more challenging to generate fixed code given that there are multi buggy lines in the buggy code.

\begin{table}[]
		\centering
	
	\fontsize{8.0}{10}\selectfont 
	\caption{Performance of Program Repair task. }
	\label{tab:program_repair}
	\begin{tabular}{ccccc}
		\hline
		\multirow{2}{*}{Baselines} & \multicolumn{2}{c}{SL-Java} & \multicolumn{2}{c}{ML-Python} \\ \cline{2-5} 
		& EM           & BLEU         & EM            & BLEU          \\ \hline
		CodeBERT                   & 3.66         & 34.21        & 2.40          & 29.40         \\
		GraphCodeBERT              & 3.35         & 35.29        & 3.31          & 30.59         \\
		PLBART                     & 6.02         & 40.12        & 4.01          & 33.92         \\ \hline
		CodeT5 (PR objective)      & 8.41         & 40.20        & 4.62          & 35.52         \\
		CodeT5 (all objectives)    & 13.30        & 43.42        & 5.30          & 38.85         \\ \hline
	\end{tabular}
\end{table}



==> introduction.tex <==
%!TEX root=emnlp2022.tex
% \begin{figure*}[t]
% 	\centering
% 	\includegraphics[scale=.25]{figures/overview2.png}
% 	\caption{An overview of our framework  }
% 	\label{fig:overview}
% \end{figure*}


Program debugging is an important task in software engineering. The goal of program debugging is to localize buggy locations of the program (bug localization) and fixes such buggy locations (program repair).
The majority of debugging tools fall into two categories: program analysis-based and neural-based. To debug a program, program analysis-based techniques employ compiler-based and software engineering theory to build code analysis tools. These methods have a significant disadvantage in that they are not scalable to large programs.
On the other hand, a recent trend is to use neural-based techniques~\cite{lutellier2020coconut, jiang2021cure,zhu2021syntax,mashhadi2021applying,ding2020patching, wang2021codet5} are based on the \textit{naturalness hypothesis }of software code~\cite{hindle2016naturalness}. These techniques rely on large code corpora that can be used as training and test sets, allowing machine learning methods to learn and probabilistically reason about coding practice on a large scale. The goal is to develop useful tools on top of these models  and program debugging is one of the topics that has received a lot of attention in order to employ such neural-based model to build such tools. 

Existing neural-based program debugging techniques have three major flaws.
To begin, the majority of the techniques work by utilising unique source code features such as control flow, data flow, abstract syntax trees, and so on. However, to extract source code features, these techniques necessitate careful design of code representations and a significant amount of engineering effort, limiting their applicability to specific domains or programming languages. Second, recent studies have focused on detecting bugs at coarse-grained code granularity (function level or file level)
According to recent surveys~\cite{zou2019empirical} on the adoption of such tools in real-world use, this is not a very useful signal for developers. Buggy signals should be provided by the tools at finer-grained code levels, such as the statement, line, or token level. The neural-based bug detection tool at the token level, on the other hand, is said to be too fine-grained and generate a large number of false positives, rendering the tool useless~\cite{allamanis2021self}. The line level is the most reasonable level of bug detection because it corresponds to how the developer reads and debugs programs. Finally, these techniques are only intended for bug localization or program repair, whereas a good program debugging tool should be capable of both.

To address the issues above, we propose a unified framework for fine-tuning pretrained language models of code for program debugging, including 3 tasks: function-level bug detection, line-level bug detection and program repair.  Using code pretrained language models has two advantages. First, by treating code as natural language, it reduces the effort of the code representation process. Second, it can apply the knowledge gained from the pretrained step on large-scale datasets. We use CodeT5~\cite{wang2021codet5} as the foundation model because it is the state-of-the-art model for many code learning tasks, and it has been pretrained on code-aware features such as identifiers, function names, and code documentation, allowing the model to understand source code better than other models. 
The main idea is to fine-tune CodeT5 on three objectives that are specifically designed for code. The first objective is the function-level bug detection task, which is to detect if a given code contains bug or not. Second, to provide more useful information to developer at finer-grained code granularity, we introduce a line ranking objective to rank the lines in in the code snippet according to some scores. Finally, we employ an additional patch generation objective to translate the buggy code to correct code (if any)~\footnote{Patch generation refers to the process of creating the correct fix for a buggy code snippet.}. These 3 objectives complement on each other and each will assist the others to make the overall performance better.

We trained our model based on the datasets of bug-fixing code changes collected on Github. Once trained,
We evaluate our models for 4 separate tasks: function-level bug detection, line-level bug detection, program repair and a unify program-debugging task.  Our evaluation shows that our model perform the best among the baselines for all of the tasks. We also conduct additional ablation studies to demonstrate that training the three objectives concurrently improves performance significantly more than training each task separately. Finally, we perform a unify evaluation task that mimic how developers localize and fix bugs. This is to evaluate how well our model performs in real-world scenario when a developer needs to debug a program.

Our contribution can be summazired as:
~\begin{enumerate}[leftmargin=*]
	\item We propose a unify framework with 3 objectives that solve program debugging related tasks: function-level bug localization objective, line ranking objective and patch generation objective.
	\item We introduce new large-scale datasets in 2 programming languages (Java and Python) with useful information for future research, including the buggy line indicator; and the before-fixed version and the after-fixed version of code snippets.
	\item We perform extensive evaluation on 4 tasks function-level bug detection, line-level bug detection, program repair and a unify program-debugging task and shows that our model outperform the other baselines with significant margin.
\end{enumerate}




==> model_new.tex <==
\section{Approach}
\label{sec:model}
As shown in Figure~\ref{fig:overview}, we present a unified framework to jointly address three crucial tasks in bug fixing: \emph{bug detection} (whether a given code snippet contains bugs), \emph{bug localization} (which lines are buggy), and \emph{program repair} (how to repair bugs).
We first define the input/output formulation of these tasks in \S~\ref{ssec:formulation} and then revisit our foundation model CodeT5 in \S~\ref{ssec:codet5}, followed by introducing each of tasks in \S~\ref{ssec:localize_repair} in details.


\begin{figure*}[t]
	\centering
	\includegraphics[width=0.99\textwidth]{figures/codet5_bug_locator.pdf}
	\caption{An overview of our framework}
	\label{fig:overview}
\end{figure*}


\subsection{Input and Output} \label{ssec:formulation}
Let $\mathcal{D}$ be a program repair dataset consisting of $|\mathcal{D}|$  triplets of $(X,Y,F)$. $X$ is the source program patch at function level and $Y=\{y_1, ..., y_L\}$ is its buggy labels for each line, where $y_i \in [0,1]$ represents whether the $i$-th line is buggy or not and $L$ denotes the number of lines in $X$. $F$ is the target fixed program if source patch $X$ contains any buggy lines, otherwise it is an empty string. Let $y$ denote such function-level binary label and $y=1$ if there exists $y_i=1$ and else $y=0$.
For the input format of $X$, we insert a special token \texttt{[SEP]} for each line to inform the end of line information. 

\subsection{Revisit CodeT5} \label{ssec:codet5}
CodeT5~\cite{wang2021codet5} is a unified pretrained encoder-decoder language models for code. It was pretrained on a large-scale source code corpus collected from Github which consists of 8 different programming languages (including Java and Python). Moreover, CodeT5 proposed an identifier-aware pretraining objective to endow the model with code-specific knowledge. Besides that, it employs a code-specific Byte-Pair Encoding (BPE)~\cite{DBLP:conf/acl/SennrichHB16a} tokenizer that is able to avoid Out-of-Vocabulary (OoV) problems. CodeT5 has achieved state-of-the-art (SOTA) performance on a wide range of code intelligence tasks in CodeXGLUE~\cite{lu2021codexglue} such as defect detection and code refinement. In this work, we adapt CodeT5 as our foundation model and propose a new unified framework to jointly solve bug localization and repair.

\subsection{Bug Localization and Repair} \label{ssec:localize_repair}
In this subsection, we introduce how to adapt CodeT5 for bug detection, localization, and repair. 

\paragraph{Function-Level Bug Detection} \label{ssec:fbd}
The goal of this task is to detect whether a function contains any bugs. Given an input code patch $X$, we aim to learn the binary probability of $P_{\theta}(y|X)$ with CodeT5 parameterized by $\theta$. Specifically, we pass the source patch $X$ to both encoder and decoder of CodeT5 and adopt the last decoder state as the sequence representation of $X$, followed by a linear layer on top of it for a binary classification. This task is optimized with a standard cross entropy loss in training and a patch is considered as buggy if the predicted probability is higher than a threshold of $0.5$ in inference.

\paragraph{Line-Level Bug Localization} \label{ssec:lbd}
A further step of bug detection is to localize which exact lines are buggy. This is an important intermediate task for the final successful repair. This task is formulated to compute $P_{\phi}(Y|X)$, which $\phi$ denotes the parameter of the encoder of CodeT5. Specifically, we gather the last layer states of all \texttt{[SEP]} tokens from the encoder and map them to a vector of probabilities $\hat{Y}=\{\hat{y}_1, ..., \hat{y}_L\}$. We approach the bug localization as a sequence labeling task and apply the binary cross entropy loss between $\hat{Y}$ and $Y$ during training. For inference, we obtain the top-$k$ predictions and measure how they match the ground truth with retrieval metrics. Notable, we consider two settings of bug localization where the source patch can  have only one single buggy line or multiple buggy lines.

\paragraph{Program Repair} \label{ssec:apr}
This task aims to translate a buggy source patch $X$ into its fixed version $F$. Formally, we aim to learn the probability
$P_{\theta}(F|X)=\prod_{j=1}^{n}P_{\theta}(Y_j| X,F_1:F_j-1)$, where $F_1:F_j-1$ is the previous sequence before the $j$-th token and $n$ denotes the number of tokens in the target sequence $F$. We approach this task a sequence-to-sequence problem and train with a standard sequence generation loss. During inference, we adopt beam search to generate a ranked list of fixed candidate patches.

During training, we adopt multi-task learning to simultaneously optimize these three tasks in an end-to-end manner. The intuition behind this design is that these tasks are highly related and can  complement to each other, e.g., a preciser bug locator can better inform the repairer with bug location to aid the bug fixing. Therefore, we expect these tasks can benefit from such joint training.



==> sections/model.tex <==
%!TEX root=emnlp2022.tex

Figure~\ref{fig:overview} shows an overview of our framework. 
First, from the buggy code snippet (before), we replace all of the line break with a special token <sep> . This is to inform the model that such token represents lines in the code snippet. The code snippet is then tokenized into sub-tokens and fed into the pretrained CodeT5. After going through CodeT5, we filtered the token representations and used the token representations <sep> for the Line Labeling Objective. The Line Labeling Objective's goal is to predict the label of the tokens <sep> (0 or 1), which implies detecting whether or not a line is buggy. As an auxiliary task for the Line Labeling Objective, we use another Patch Generation Objective to translate the buggy code snippet to the fixed code snippet.

\subsection{Problem Formulation}

%Given a $\mathcal{C}$
%
\subsection{Bug Detection Objective}
%The goal of this objective is to detect if a given code snippet $\mathcal{C}$ is buggy or not.  The output of the encoder of CodeT5 will go through a feed forward layer $f(.)$ and get an output $\hat{y}$. Then a sigmoid function is use to classify $\hat{y}$. The loss function is defined as binary cross-entropy.
%

%\begin{equation}
%	\small
%\mathcal{L}(\Theta, \hat{y},y) = \sum(-(y.(log(\hat{y}) + (1-y).log(1-\hat{y})))
%\end{equation}\\
%\subsection{Line Ranking Objective}
%%We construct a sequence of binary labels $y\in\left\{0,1\right\}$ for the special token\texttt{ <sep>} to indicate if a line is buggy or not . However, we use the KL-digervence loss to compare the 2 distributions with the goal. We will clarify our design choice

\subsection{Line Ranking Objective}

\subsection{Patch Generation Objective}


